A review of simulation and performance modeling for the Roman coronagraph instrument

The Nancy Grace Roman Space Telescope Coronagraph Instrument (CGI) will be capable of characterizing exoplanets in reflected light and will demonstrate space technologies essential for future missions to take spectra of Earthlike exoplanets. As the mission and instrument move into the final stages of design, simulation tools spanning from depth of search calculators to detailed diffraction models have been created by a variety of teams. We summarize these efforts, with a particular focus on publicly available datasets and software tools. These include speckle and point-spread-function models, signal-to-noise calculators, and science product simulations (e.g. predicted observations of debris disks and exoplanet spectra). This review is intended to serve as a reference to facilitate engagement with the technical and science capabilities of the CGI instrument.

==> table_only.tex <==

\begin{table}[ht]
\renewcommand*{\arraystretch}{1.5}
    \centering
    \caption{Open Source CGI Software Packages}
    \label{tab:my_label}
    \footnotesize
    \begin{tabular}{L{3.75cm}|L{3.75cm}|c|p{6.25cm}}
    \hline
    Package & Application & References & URL\\
    \hline
    Observing Scenarios    & Complete observation simulation  & \citenum{krist_numerical_2015}& \url{https://roman.ipac.caltech.edu/sims/Coronagraph_public_images.html}\\
    PROPER & Diffraction simulation & \cite{krist_proper:_2007,krist_wfirst_2017} & \url{https://github.com/ajeldorado/proper-models/tree/master/wfirst_cgi}\\
     \verb+FALCO+  & Diffraction simulation   & \citenum{riggs2018falco1} & \url{https://github.com/ajeldorado/falco-matlab} \\
     Lightweight Coronagraph Simulator & Coronagraph Simulation & \citenum{pogorelyuk_effects_2020}& \url{https://github.com/leonidprinceton/LightweightSpaceCoronagraphSimulator}\\
     CZT-based Optical Propagation & Diffraction Simulation && \url{https://github.com/ARCExoplanetTechnologies/OpticalPropagation}\\
           \verb+WebbPSF+ & Diffraction Simulation & \citenum{perrin_simulating_2012,perrin_updated_2014}  & \url{https://github.com/spacetelescope/webbpsf}\\

     MSWC & Binary Star Simulation & \citenum{dsirbu2017mswc,dsirbu2018RomanMSWC} & \url{https://github.com/ARCExoplanetTechnologies/MSWC}\\
     \verb+EXOSIMS+ & Mission Simulation & \citenum{savransky_exosims_2017,savransky_wfirst-afta_2016} &\url{https://github.com/dsavransky/EXOSIMS}\\
     Imaging Mission Database&Mission Planning&\citenum{savransky_exploration_2019} & \url{https://plandb.sioslab.com}\\
     Coronagraph convolved Debris Disks & Disk Simulation & \citenum{mennesson_wfirst_2018}& \url{https://roman.ipac.caltech.edu/sims/Circumstellar_Disk_Sims.html} \\
     Known debris disk simulated scenes & Disk Simulation &\citenum{chen_wfirst_nodate}&  \url{https://roman.ipac.caltech.edu/sims/Chen_WPS.html}\\
     direct-imaging-sims + model spectra & Target simulation &\citenum{lacy_characterization_2019, lacy_prospects_2020}  & \url{https://github.com/blacy/direct-imaging-sims},
    \url{https://www.astro.princeton.edu/~burrows/wfirst/index.html}\\
         Giant planet albedo spectra & Target simulation & \citenum{cahoy_exoplanet_2010}  &  \url{https://wfirst.ipac.caltech.edu/sims/Exoplanet_Characterization.html}\\
     \hline
    \end{tabular}
\end{table}

